NeuroPlug: Plugging Side-Channel Leaks in NPUs using Space Filling Curves

Securing deep neural networks (DNNs) from side-channel attacks is an important problem as of today, given the substantial investment of time and resources in acquiring the raw data and training complex models. All published countermeasures (CMs) add noise N to a signal X (parameter of interest such as the net memory traffic that is leaked). The adversary observes X+N ; we shall show that it is easy to filter this noise out using targeted measurements, statistical analyses and different kinds of reasonably-assumed side information. We present a novel CM NeuroPlug that is immune to these attack methodologies mainly because we use a different formulation CX + N . We introduce a multiplicative variable C that naturally arises from feature map compression; it plays a key role in obfuscating the parameters of interest. Our approach is based on mapping all the computations to a 1-D space filling curve and then performing a sequence of tiling, compression and binning-based obfuscation operations. We follow up with proposing a theoretical framework based on Mellin transforms that allows us to accurately quantify the size of the search space as a function of the noise we add and the side information that an adversary possesses. The security guarantees provided by NeuroPlug are validated using a battery of statistical and information theory-based tests. We also demonstrate a substantial performance enhancement of 15% compared to the closest competing work.

==> ref.tex <==
https://github.com/johnrachwan123/Early-Cropression-via-Gradient-Flow-Preservation
@inproceedings{deepsniffer,
  title={Deepsniffer: A dnn model extraction framework based on learning architectural hints},
  author={Hu, Xing and Liang, Ling and Li, Shuangchen and Deng, Lei and Zuo, Pengfei and Ji, Yu and Xie, Xinfeng and Ding, Yufei and Liu, Chang and Sherwood, Timothy and others},
  booktitle={Proceedings of the Twenty-Fifth International Conference on Architectural Support for Programming Languages and Operating Systems},
  pages={385--399},
  year={2020}
}

@inproceedings{neurounlock,
  title={NeuroUnlock: Unlocking the Architecture of Obfuscated Deep Neural Networks},
  author={Ahmadi, Mahya Morid and Alrahis, Lilas and Colucci, Alessio and Sinanoglu, Ozgur and Shafique, Muhammad},
  booktitle={2022 International Joint Conference on Neural Networks (IJCNN)},
  pages={01--10},
  year={2022},
  organization={IEEE}
}

@inproceedings{huffduff,
  title={HuffDuff: Stealing Pruned DNNs from Sparse Accelerators},
  author={Yang, Dingqing and Nair, Prashant J and Lis, Mieszko},
  booktitle={Proceedings of the 28th ACM International Conference on Architectural Support for Programming Languages and Operating Systems, Volume 2},
  pages={385--399},
  year={2023}
}

@inproceedings{reverse,
  title={Reverse engineering convolutional neural networks through side-channel information leaks},
  author={Hua, Weizhe and Zhang, Zhiru and Suh, G Edward},
  booktitle={Proceedings of the 55th Annual Design Automation Conference},
  pages={1--6},
  year={2018}
}


@inproceedings{oram1,
  title={Imbalance-aware scheduler for fast and secure ring oram data retrieval},
  author={Che, Yuezhi and Hong, Yuan and Wang, Rujia},
  booktitle={2019 IEEE 37th International Conference on Computer Design (ICCD)},
  pages={604--612},
  year={2019},
  organization={IEEE}
}

@inproceedings{oram2,
  title={Multi-range supported oblivious RAM for efficient block data retrieval},
  author={Che, Yuezhi and Wang, Rujia},
  booktitle={2020 IEEE International Symposium on High Performance Computer Architecture (HPCA)},
  pages={369--382},
  year={2020},
  organization={IEEE}
}

@inproceedings{tnpu,
  title={TNPU: Supporting trusted execution with tree-less integrity protection for neural processing unit},
  author={Lee, Sunho and Kim, Jungwoo and Na, Seonjin and Park, Jongse and Huh, Jaehyuk},
  booktitle={2022 IEEE International Symposium on High-Performance Computer Architecture (HPCA)},
  pages={229--243},
  year={2022},
  organization={IEEE}
}


@inproceedings{guardnn,
  title={GuardNN: secure accelerator architecture for privacy-preserving deep learning},
  author={Hua, Weizhe and Umar, Muhammad and Zhang, Zhiru and Suh, G Edward},
  booktitle={Proceedings of the 59th ACM/IEEE Design Automation Conference},
  pages={349--354},
  year={2022}
}


@inproceedings{securator,
  title={Securator: A Fast and Secure Neural Processing Unit},
  author={Shrivastava, Nivedita and Sarangi, Smruti Ranjan},
  booktitle={2023 IEEE International Symposium on High-Performance Computer Architecture (HPCA)},
  pages={1127--1139},
  year={2023},
  organization={IEEE}
}

 @inproceedings{slalom,
  title={Slalom: Fast, Verifiable and Private Execution of Neural Networks in Trusted Hardware},
  author={Tramer, Florian and Boneh, Dan},
  booktitle={ICLR},
  year={2018}
}

@inproceedings{hybridtee,
  title={HybridTEE: Secure Mobile DNN Execution Using Hybrid Trusted Execution Environment},
  author={Gangal, Akshay and Ye, Mengmei and Wei, Sheng},
  booktitle={AsianHOST},
  pages={1--6},
  year={2020},
  organization={IEEE}
}

@inproceedings{darknight,
  title={DarKnight: An accelerated framework for privacy and integrity preserving deep learning using trusted hardware},
  author={Hashemi, Hanieh and Wang, Yongqin and Annavaram, Murali},
  booktitle={MICRO-54},
  pages={212--224},
  year={2021}
}

@inproceedings{vessels,
  title={Vessels: efficient and scalable deep learning prediction on trusted processors},
  author={Kim, Kyungtae and Kim, Chung Hwan and Rhee, Junghwan" John" and Yu, Xiao and Chen, Haifeng and Tian, Dave and Lee, Byoungyoung},
  booktitle={SoCC},
  pages={462--476},
  year={2020}
}

@article{esl,
  title={Towards an Optimal Countermeasure for Cache Side-Channel Attacks},
  author={Shrivastava, Nivedita and Sarangi, Smruti R},
  journal={IEEE Embedded Systems Letters},
  year={2022},
  publisher={IEEE}
}

@inproceedings{cachetelepathy,
  title={Cache telepathy: Leveraging shared resource attacks to learn DNN architectures},
  author={Yan, Mengjia and Fletcher, Christopher and Torrellas, Josep},
  booktitle={USENIX Security Symposium},
  year={2020}
}

@inproceedings{ceaser,
  title={CEASER: Mitigating conflict-based cache attacks via encrypted-address and remapping},
  author={Qureshi, Moinuddin K},
  booktitle={2018 51st Annual IEEE/ACM International Symposium on Microarchitecture (MICRO)},
  pages={775--787},
  year={2018},
  organization={IEEE}
}

@inproceedings{scattercache,
  title={ScatterCache: Thwarting Cache Attacks via Cache Set Randomization.},
  author={Werner, Mario and Unterluggauer, Thomas and Giner, Lukas and Schwarz, Michael and Gruss, Daniel and Mangard, Stefan},
  booktitle={USENIX Security Symposium},
  pages={675--692},
  year={2019}
}


@article{survey,
  title={A survey of convolutional neural networks: analysis, applications, and prospects},
  author={Li, Zewen and others},
  journal={IEEE trans. on  neural netw learn syst},
  year={2021},
  publishr={IEEE}
}

@article{eyerissv2,
  title={Eyeriss v2: A flexible accelerator for emerging deep neural networks on mobile devices},
  author={Chen, Yu-Hsin and Yang, Tien-Ju and Emer, Joel and Sze, Vivienne},
  journal={IEEE Journal on Emerging and Selected Topics in Circuits and Systems},
  volume={9},
  number={2},
  pages={292--308},
  year={2019},
  publisher={IEEE}
}

@article{scnn,
  title={SCNN: An accelerator for compressed-sparse convolutional neural networks},
  author={Parashar, Angshuman and Rhu, Minsoo and Mukkara, Anurag and Puglielli, Antonio and Venkatesan, Rangharajan and Khailany, Brucek and Emer, Joel and Keckler, Stephen W and Dally, William J},
  journal={ACM SIGARCH computer architecture news},
  volume={45},
  number={2},
  pages={27--40},
  year={2017},
  publisher={ACM New York, NY, USA}
}

@article{fsa,
  title={Fsa: A fine-grained systolic accelerator for sparse cnns},
  author={Li, Fanrong and Li, Gang and Mo, Zitao and He, Xiangyu and Cheng, Jian},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={39},
  number={11},
  pages={3589--3600},
  year={2020},
  publisher={IEEE}
}

@inproceedings{sparten,
  title={SparTen: A sparse tensor accelerator for convolutional neural networks},
  author={Gondimalla, Ashish and Chesnut, Noah and Thottethodi, Mithuna and Vijaykumar, TN},
  booktitle={Proceedings of the 52nd Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={151--165},
  year={2019}
}

@article{swallow,
  title={Swallow: A versatile accelerator for sparse neural networks},
  author={Liu, Bosheng and Chen, Xiaoming and Han, Yinhe and Xu, Haobo},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={39},
  number={12},
  pages={4881--4893},
  year={2020},
  publisher={IEEE}
}


@article{mayer2006fisher,
  title={Fisher information and dynamic regime changes in ecological systems},
  author={Mayer, Audrey L and Pawlowski, Christopher W and Cabezas, Heriberto},
  journal={Ecological modelling},
  volume={195},
  number={1-2},
  pages={72--82},
  year={2006},
  publisher={Elsevier}
}

@inproceedings{kayhan2020translation,
  title={On translation invariance in cnns: Convolutional layers can exploit absolute spatial location},
  author={Kayhan, Osman Semih and Gemert, Jan C van},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={14274--14285},
  year={2020}
}


@article{ahmad2016using,
  title={Using Fisher information to track stability in multivariate systems},
  author={Ahmad, Nasir and Derrible, Sybil and Eason, Tarsha and Cabezas, Heriberto},
  journal={Royal Society open science},
  volume={3},
  number={11},
  pages={160582},
  year={2016},
  publisher={The Royal Society}
}

@article{karunanithi2008detection,
  title={Detection and assessment of ecosystem regime shifts from Fisher information},
  author={Karunanithi, Arunprakash T and Cabezas, Heriberto and Frieden, B Roy and Pawlowski, Christopher W},
  journal={Ecology and society},
  volume={13},
  number={1},
  year={2008},
  publisher={JSTOR}
}


@article{scedl,
  title={SceDL: A Simultaneous Compression and Encryption Scheme for Deep Learning Models},
  author={Shrivastava, Nivedita and others},
  year={2023},
  publisher={TechRxiv}
}

@inproceedings{bdi,
  title={Base-delta-immediate compression: Practical data compression for on-chip caches},
  author={Pekhimenko, Gennady and Seshadri, Vivek and Mutlu, Onur and Gibbons, Phillip B and Kozuch, Michael A and Mowry, Todd C},
  booktitle={Proceedings of the 21st international conference on Parallel architectures and compilation techniques},
  pages={377--388},
  year={2012}
}

@article{cpack,
  title={C-pack: A high-performance microprocessor cache compression algorithm},
  author={Chen, Xi and Yang, Lei and Dick, Robert P and Shang, Li and Lekatsas, Haris},
  journal={IEEE transactions on very large scale integration (VLSI) systems},
  volume={18},
  number={8},
  pages={1196--1208},
  year={2009},
  publisher={IEEE}
}

@techreport{fpc,
  title={Frequent pattern compression: A significance-based compression scheme for L2 caches},
  author={Alameldeen, Alaa and Wood, David},
  year={2004},
  institution={University of Wisconsin-Madison Department of Computer Sciences}
}

@misc{zstd,
  title={Zstd github repository from facebook},
  author={Collet, Y},
  year={2016}
}

@article{huffman,
  title={A method for the construction of minimum-redundancy codes},
  author={Huffman, David A},
  journal={Proceedings of the IRE},
  volume={40},
  number={9},
  pages={1098--1101},
  year={1952},
  publisher={IEEE}
}

@inproceedings{lamp,
title={Layer-adaptive Sparsity for the Magnitude-based Pruning},
author={Jaeho Lee and Sejun Park and Sangwoo Mo and Sungsoo Ahn and Jinwoo Shin},
booktitle={International Conference on Learning Representations},
year={2021},
url={https://openreview.net/forum?id=H6ATjJ0TKdf}
}

@article{zlib,
  title={Zlib compression library},
  author={Gailly, Jean-loup and Adler, Mark},
  year={2004}
}


@article{eyeriss,
  title={Eyeriss: An energy-efficient reconfigurable accelerator for deep convolutional neural networks},
  author={Chen, Yu-Hsin and Krishna, Tushar and Emer, Joel S and Sze, Vivienne},
  journal={IEEE journal of solid-state circuits},
  volume={52},
  number={1},
  pages={127--138},
  year={2016},
  publisher={IEEE}
}


@inproceedings{Ttrace,
  title={Hardware Abstractions for targeting EDDO Architectures with the Polyhedral Model},
  author={Parashar, Angshuman and Chatarasi, Prasanth and Tsai, Po-An},
  booktitle={11th International Workshop on Polyhedral Compilation Techniques (Vitural Event)(IMPACT 2021)},
  year={2021}
}

@inproceedings{timeloop,
  title={Timeloop: A systematic approach to dnn accelerator evaluation},
  author={Parashar, Angshuman and Raina, Priyanka and Shao, Yakun Sophia and Chen, Yu-Hsin and Ying, Victor A and Mukkara, Anurag and Venkatesan, Rangharajan and Khailany, Brucek and Keckler, Stephen W and Emer, Joel},
  booktitle={2019 IEEE international symposium on performance analysis of systems and software (ISPASS)},
  pages={304--315},
  year={2019},
  organization={IEEE}
}

@article{ramulator,
  title={Ramulator: A fast and extensible DRAM simulator},
  author={Kim, Yoongu and Yang, Weikun and Mutlu, Onur},
  journal={IEEE Computer architecture letters},
  volume={15},
  number={1},
  pages={45--49},
  year={2015},
  publisher={IEEE}
}

@inproceedings{MIleakage,
  title={Leakage assessment through neural estimation of the mutual information},
  author={Cristiani, Valence and Lecomte, Maxime and Maurine, Philippe},
  booktitle={Applied Cryptography and Network Security Workshops: ACNS 2020 Satellite Workshops, AIBlock, AIHWS, AIoTS, Cloud S\&P, SCI, SecMT, and SiMLA, Rome, Italy, October 19--22, 2020, Proceedings 18},
  pages={144--162},
  year={2020},
  organization={Springer}
}

@inproceedings{MIleakage2,
  title={Making masking security proofs concrete: or how to evaluate the security of any leaking device},
  author={Duc, Alexandre and Faust, Sebastian and Standaert, Fran{\c{c}}ois-Xavier},
  booktitle={Advances in Cryptology--EUROCRYPT 2015: 34th Annual International Conference on the Theory and Applications of Cryptographic Techniques, Sofia, Bulgaria, April 26-30, 2015, Proceedings, Part I 34},
  pages={401--429},
  year={2015},
  organization={Springer}
}

@inproceedings{MI3,
  title={Statistical measurement of information leakage},
  author={Chatzikokolakis, Konstantinos and Chothia, Tom and Guha, Apratim},
  booktitle={International Conference on Tools and Algorithms for the Construction and Analysis of Systems},
  pages={390--404},
  year={2010},
  organization={Springer}
}

@inproceedings{MI4,
  title={Theoretical and practical aspects of mutual information based side channel analysis},
  author={Prouff, Emmanuel and Rivain, Matthieu},
  booktitle={Applied Cryptography and Network Security: 7th International Conference, ACNS 2009, Paris-Rocquencourt, France, June 2-5, 2009. Proceedings 7},
  pages={499--518},
  year={2009},
  organization={Springer}
}

@article{MI5,
  title={Best information is most successful},
  author={De Ch{\'e}risey, Eloi and Guilley, Sylvain and Rioul, Olivier and Piantanida, Pablo},
  journal={Cryptology ePrint Archive},
  year={2019}
}


@inproceedings{fisher1,
  title={Fisher information determines capacity of $\varepsilon$-secure steganography},
  author={Filler, Tom{\'a}{\v{s}} and Fridrich, Jessica},
  booktitle={International Workshop on Information Hiding},
  pages={31--47},
  year={2009},
  organization={Springer}
}
@article{fisher2,
  title={Modelling and quantifying membership information leakage in machine learning},
  author={Farokhi, Farhad and Kaafar, Mohamed Ali},
  journal={arXiv preprint arXiv:2001.10648},
  year={2020}
}
@inproceedings{fisher3,
  title={Measuring data leakage in machine-learning models with Fisher information},
  author={Hannun, Awni and Guo, Chuan and van der Maaten, Laurens},
  booktitle={Uncertainty in Artificial Intelligence},
  pages={760--770},
  year={2021},
  organization={PMLR}
}

@article{fisher4,
  title={Measuring and Controlling Split Layer Privacy Leakage Using Fisher Information},
  author={Maeng, Kiwan and Guo, Chuan and Kariyappa, Sanjay and Suh, Edward},
  journal={arXiv preprint arXiv:2209.10119},
  year={2022}
}

@article{fisher5,
  title={Cramer-Rao lower bound for performance analysis of leak detection},
  author={Keramat, Alireza and Ghidaoui, Mohamed S and Wang, Xun and Louati, Moez},
  journal={Journal of Hydraulic Engineering},
  volume={145},
  number={6},
  pages={04019018},
  year={2019},
  publisher={American Society of Civil Engineers}
}




@article{CVM1,
  title={A new ECDF two-sample test statistic},
  author={Dowd, Connor},
  journal={arXiv preprint arXiv:2007.01360},
  year={2020}
}


@article{CVM2,
  title={Cram{\'e}r--von Mises distance: probabilistic interpretation, confidence intervals, and neighbourhood-of-model validation},
  author={Baringhaus, L and Henze, N},
  journal={Journal of Nonparametric Statistics},
  volume={29},
  number={2},
  pages={167--188},
  year={2017},
  publisher={Taylor \& Francis}
}

@article{CVM3,
  title={Cram{\'e}r-von Mises statistics for discrete distributions},
  author={Choulakian, Vartan and Lockhart, Richard A and Stephens, Michael A},
  journal={The Canadian Journal of Statistics/La Revue Canadienne de Statistique},
  pages={125--137},
  year={1994},
  publisher={JSTOR}
}

@article{lane,
  title={Lane compression: A lightweight lossless compression method for machine learning on embedded systems},
  author={Ko, Yousun and Chadwick, Alex and Bates, Daniel and Mullins, Robert},
  journal={ACM Transactions on Embedded Computing Systems (TECS)},
  volume={20},
  number={2},
  pages={1--26},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@article{rle,
  title={Run-length encodings (corresp.)},
  author={Golomb, Solomon},
  journal={IEEE transactions on information theory},
  volume={12},
  number={3},
  pages={399--401},
  year={1966},
  publisher={Citeseer}
}

@inproceedings{ebpc,
  title={Extended bit-plane compression for convolutional neural network accelerators},
  author={Cavigelli, Lukas and Benini, Luca},
  booktitle={2019 IEEE International Conference on Artificial Intelligence Circuits and Systems (AICAS)},
  pages={279--283},
  year={2019},
  organization={IEEE}
}

@article{sparsity,
  title={Going deeper in spiking neural networks: VGG and residual architectures},
  author={Sengupta, Abhronil and Ye, Yuting and Wang, Robert and Liu, Chiao and Roy, Kaushik},
  journal={Frontiers in neuroscience},
  volume={13},
  pages={95},
  year={2019},
  publisher={Frontiers Media SA}
}

@misc{resnet_pretrain,
  title = {{MS Windows NT} Kernel Description},
  howpublished = {\url{https://pytorch.org/vision/stable/models/generated/torchvision.models.resnet18.html#torchvision.models.resnet18}},
  note = {Accessed: 2023-07-20}
}

@misc{vgg_pretrain,
  title = {{MS Windows NT} Kernel Description},
  howpublished = {\url{https://pytorch.org/vision/stable/models/generated/torchvision.models.vgg16.html#torchvision.models.vgg16}},
  note = {Accessed: 2023-07-20}
}
%https://pytorch.org/vision/stable/models/generated/torchvision.models.vgg16.html#torchvision.models.vgg16
%https://pytorch.org/vision/stable/models/generated/torchvision.models.resnet18.html#torchvision.models.resnet18

@inproceedings{resnet,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}
@article{vggnet,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}


@inproceedings{sealing,
  title={Sealing neural network models in encrypted deep learning accelerators},
  author={Zuo, Pengfei and Hua, Yu and Liang, Ling and Xie, Xinfeng and Hu, Xing and Xie, Yuan},
  booktitle={2021 58th ACM/IEEE Design Automation Conference (DAC)},
  pages={1255--1260},
  year={2021},
  organization={IEEE}
}


@inproceedings{qd,
  title={QD-Compressor: a Quantization-based Delta Compression Framework for Deep Neural Networks},
  author={Zhang, Shuyu and Wu, Donglei and Jin, Haoyu and Zou, Xiangyu and Xia, Wen and Huang, Xiaojia},
  booktitle={2021 IEEE 39th International Conference on Computer Design (ICCD)},
  pages={542--550},
  year={2021},
  organization={IEEE}
}


@inproceedings{criticalpath,
  title={Supporting compressed-sparse activations and weights on SIMD-like accelerator for sparse convolutional neural networks},
  author={Lin, Chien-Yu and Lai, Bo-Cheng},
  booktitle={2018 23rd Asia and South Pacific Design Automation Conference (ASP-DAC)},
  pages={105--110},
  year={2018},
  organization={IEEE}
}

@inproceedings{CSRmultiplication,
  title={Parallel sparse matrix-vector and matrix-transpose-vector multiplication using compressed sparse blocks},
  author={Bulu{\c{c}}, Aydin and Fineman, Jeremy T and Frigo, Matteo and Gilbert, John R and Leiserson, Charles E},
  booktitle={Proceedings of the twenty-first annual symposium on Parallelism in algorithms and architectures},
  pages={233--244},
  year={2009}
}

@article{membership,
  title={Understanding membership inferences on well-generalized learning models},
  author={Long, Yunhui and Bindschaedler, Vincent and Wang, Lei and Bu, Diyue and Wang, Xiaofeng and Tang, Haixu and Gunter, Carl A and Chen, Kai},
  journal={arXiv preprint arXiv:1802.04889},
  year={2018}
}

@inproceedings{stealing,
  title={Stealing machine learning models via prediction APIs},
  author={Tramer, Florian and Zhang, Fan and Juels, Ari and Reiter, Michael K and Ristenpart, Thomas},
  booktitle={25th USENIX security symposium (USENIX Security 16)},
  pages={601--618},
  year={2016}
}

@article{adversarial,
  title={Delving into transferable adversarial examples and black-box attacks},
  author={Liu, Yanpei and Chen, Xinyun and Liu, Chang and Song, Dawn},
  journal={arXiv preprint arXiv:1611.02770},
  year={2016}
}

@article{classification,
  title={Deep neural networks with region-based pooling structures for mammographic image classification},
  author={Shu, Xin and Zhang, Lei and Wang, Zizhou and Lv, Qing and Yi, Zhang},
  journal={IEEE transactions on medical imaging},
  volume={39},
  number={6},
  pages={2246--2255},
  year={2020},
  publisher={IEEE}
}

@article{security,
  title={A survey of machine and deep learning methods for internet of things (IoT) security},
  author={Al-Garadi, Mohammed Ali and Mohamed, Amr and Al-Ali, Abdulla Khalid and Du, Xiaojiang and Ali, Ihsan and Guizani, Mohsen},
  journal={IEEE Communications Surveys \& Tutorials},
  volume={22},
  number={3},
  pages={1646--1685},
  year={2020},
  publisher={IEEE}
}

@article{automobile,
  title={Automobile driver fingerprinting: A new machine learning based authentication scheme},
  author={Xun, Yijie and Liu, Jiajia and Kato, Nei and Fang, Yongqiang and Zhang, Yanning},
  journal={IEEE Transactions on Industrial Informatics},
  volume={16},
  number={2},
  pages={1417--1426},
  year={2019},
  publisher={IEEE}
}

@article{UAV,
  title={Deep neural network based vehicle and pedestrian detection for autonomous driving: A survey},
  author={Chen, Long and Lin, Shaobo and Lu, Xiankai and Cao, Dongpu and Wu, Hangbin and Guo, Chi and Liu, Chun and Wang, Fei-Yue},
  journal={IEEE Transactions on Intelligent Transportation Systems},
  volume={22},
  number={6},
  pages={3234--3246},
  year={2021},
  publisher={IEEE}
}

@article{speech,
  title={Speech recognition using deep neural networks: A systematic review},
  author={Nassif, Ali Bou and Shahin, Ismail and Attili, Imtinan and Azzeh, Mohammad and Shaalan, Khaled},
  journal={IEEE access},
  volume={7},
  pages={19143--19165},
  year={2019},
  publisher={IEEE}
}


@incollection{runstest,
  title={A new exact runs test for randomness},
  author={Agin, Marilyn A and Godbole, Anant P},
  booktitle={Computing Science and Statistics: Statistics of Many Parameters: Curves, Images, Spatial Models},
  pages={281--285},
  year={1992},
  publisher={Springer}
}

@inproceedings{deepfreeze,
  title={Deepfreeze: Cold boot attacks and high fidelity model recovery on commercial edgeml device},
  author={Won, Yoo-Seung and Chatterjee, Soham and Jap, Dirmanto and Basu, Arindam and Bhasin, Shivam},
  booktitle={2021 IEEE/ACM International Conference On Computer Aided Design (ICCAD)},
  pages={1--9},
  year={2021},
  organization={IEEE}
}

@inproceedings{deeplaser,
  title={Practical fault attack on deep neural networks},
  author={Breier, Jakub and Hou, Xiaolu and Jap, Dirmanto and Ma, Lei and Bhasin, Shivam and Liu, Yang},
  booktitle={Proceedings of the 2018 ACM SIGSAC Conference on Computer and Communications Security},
  pages={2204--2206},
  year={2018}
}


@article{IBPP,
  title={Notes on inverse bin-packing problems},
  author={Chung, Yerim and Park, Myoung-Ju},
  journal={Information Processing Letters},
  volume={115},
  number={1},
  pages={60--68},
  year={2015},
  publisher={Elsevier}
}

@article{sgxBPP,
  title={Concealer: Sgx-based secure, volume hiding, and verifiable processing of spatial time-series datasets},
  author={Gupta, Peeyush and Mehrotra, Sharad and Sharma, Shantanu and Venkatasubramanian, Nalini and Wang, Guoxi},
  journal={arXiv preprint arXiv:2102.05238},
  year={2021}
}


@article{nist,
  title={On the interpretation of results from the NIST statistical test suite},
  author={Marton, Kinga and Suciu, Alin},
  journal={Science and Technology},
  volume={18},
  number={1},
  pages={18--32},
  year={2015}
}


@inproceedings{lenet,
  title={Accelerator implementation of lenet-5 convolution neural network based on fpga with hls},
  author={Rongshi, Dai and Yongming, Tang},
  booktitle={2019 3rd International Conference on Circuits, System and Simulation (ICCSS)},
  pages={64--67},
  year={2019},
  organization={IEEE}
}

@inproceedings{mgx,
  title={MGX: Near-zero overhead memory protection for data-intensive accelerators},
  author={Hua, Weizhe and Umar, Muhammad and Zhang, Zhiru and Suh, G Edward},
  booktitle={Proceedings of the 49th Annual International Symposium on Computer Architecture},
  pages={726--741},
  year={2022}
}

@inproceedings{deephammer,
  title={DeepHammer: Depleting the intelligence of deep neural networks through targeted chain of bit flips},
  author={Yao, Fan and Rakin, Adnan Siraj and Fan, Deliang},
  booktitle={29th USENIX Security Symposium (USENIX Security 20)},
  pages={1463--1480},
  year={2020}
}


@inproceedings{deepsteal,
  title={Deepsteal: Advanced model extractions leveraging efficient weight stealing in memories},
  author={Rakin, Adnan Siraj and Chowdhuryy, Md Hafizul Islam and Yao, Fan and Fan, Deliang},
  booktitle={2022 IEEE Symposium on Security and Privacy (SP)},
  pages={1157--1174},
  year={2022},
  organization={IEEE}
}

@article{reverse2,
  title={Reverse-engineering cnn models using side-channel attacks},
  author={Hua, Weizhe and Zhang, Zhiru and Suh, G Edward},
  journal={IEEE Design \& Test},
  volume={39},
  number={4},
  pages={15--22},
  year={2022},
  publisher={IEEE}
}

%%%%%%%%%%%%%%%%%%%%%%%5
%statistica;
@inproceedings{prada,
  title={PRADA: protecting against DNN model stealing attacks},
  author={Juuti, Mika and Szyller, Sebastian and Marchal, Samuel and Asokan, N},
  booktitle={2019 IEEE European Symposium on Security and Privacy (EuroS\&P)},
  pages={512--527},
  year={2019},
  organization={IEEE}
}

%accuracy drop
@inproceedings{hwassisted,
  title={Hardware-assisted intellectual property protection of deep learning models},
  author={Chakraborty, Abhishek and Mondai, Ankit and Srivastava, Ankur},
  booktitle={2020 57th ACM/IEEE Design Automation Conference (DAC)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}

%accuracy drop
@article{preventingDNN,
  title={Preventing DNN model IP theft via hardware obfuscation},
  author={Goldstein, Brunno F and Patil, Vinay C and Ferreira, Victor C and Nery, Alexandre S and Fran{\c{c}}a, Felipe MG and Kundu, Sandip},
  journal={IEEE Journal on Emerging and Selected Topics in Circuits and Systems},
  volume={11},
  number={2},
  pages={267--277},
  year={2021},
  publisher={IEEE}
}

%Paramerer difference
@inproceedings{differentiallyPrivate,
  title={Differentially Private Machine Learning Model against Model Extraction Attack},
  author={Cheng, Zelei and Li, Zuotian and Zhang, Jiwei and Zhang, Shuhan},
  booktitle={2020 International Conferences on Internet of Things (iThings) and IEEE Green Computing and Communications (GreenCom) and IEEE Cyber, Physical and Social Computing (CPSCom) and IEEE Smart Data (SmartData) and IEEE Congress on Cybermatics (Cybermatics)},
  pages={722--728},
  year={2020},
  organization={IEEE}
}

%Brute force
@inproceedings{protecting,
  title={Protecting Deep Neural Network Intellectual Property with Architecture-Agnostic Input Obfuscation},
  author={Olney, Brooks and Karam, Robert},
  booktitle={Proceedings of the Great Lakes Symposium on VLSI 2022},
  pages={111--115},
  year={2022}
}

%accuracy drop, KL divergence, cosine
@inproceedings{deceptiveperturbations,
  title={Defending against neural network model stealing attacks using deceptive perturbations},
  author={Lee, Taesung and Edwards, Benjamin and Molloy, Ian and Su, Dong},
  booktitle={2019 IEEE Security and Privacy Workshops (SPW)},
  pages={43--49},
  year={2019},
  organization={IEEE}
}


@article{chaos1,
  title={Cryptanalysis of image ciphers with permutation-substitution network and chaos},
  author={Chen, Junxin and Chen, Lei and Zhou, Yicong},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  volume={31},
  number={6},
  pages={2494--2508},
  year={2020},
  publisher={IEEE}
}

@article{chaos2,
  title={Cryptanalysis of image encryption scheme based on a new 1D chaotic system},
  author={Dhall, Sakshi and Pal, Saibal K and Sharma, Kapil},
  journal={Signal processing},
  volume={146},
  pages={22--32},
  year={2018},
  publisher={Elsevier}
}

@article{chaos3,
  title={Efficient and secure image encryption algorithm using a novel key-substitution architecture},
  author={Song, Yanjie and Zhu, Zhiliang and Zhang, Wei and Yu, Hai and Zhao, Yuli},
  journal={IEEE Access},
  volume={7},
  pages={84386--84400},
  year={2019},
  publisher={IEEE}
}


@article{deepobfuscation,
  title={Deepobfuscation: Securing the structure of convolutional neural networks via knowledge distillation},
  author={Xu, Hui and Su, Yuxin and Zhao, Zirui and Zhou, Yangfan and Lyu, Michael R and King, Irwin},
  journal={arXiv preprint arXiv:1806.10313},
  year={2018}
}

%accuravy
@article{deeplock,
  title={Deep-lock: Secure authorization for deep neural networks},
  author={Alam, Manaar and Saha, Sayandeep and Mukhopadhyay, Debdeep and Kundu, Sandip},
  journal={arXiv preprint arXiv:2008.05966},
  year={2020}
}

%LER
@article{dnnalias,
  title={DNN-Alias: Deep Neural Network Protection Against Side-Channel Attacks via Layer Balancing},
  author={Ahmadi, Mahya Morid and Alrahis, Lilas and Sinanoglu, Ozgur and Shafique, Muhammad},
  journal={arXiv preprint arXiv:2303.06746},
  year={2023}
}

%LER
@article{defenseagainst,
  title={Defense against ML-based Power Side-channel Attacks on DNN Accelerators with Adversarial Attacks},
  author={Yan, Xiaobei and Chang, Chip Hong and Zhang, Tianwei},
  journal={arXiv preprint arXiv:2312.04035},
  year={2023}
}
%Propagation Kernel algorithm to calculate
the similarity between two graphs
@article{modelobfuscator,
  title={ModelObfuscator: Obfuscating Model Information to Protect Deployed ML-based Systems},
  author={Zhou, Mingyi and Gao, Xiang and Wu, Jing and Grundy, John and Chen, Xiao and Chen, Chunyang and Li, Li},
  journal={arXiv preprint arXiv:2306.06112},
  year={2023}
}

%accu drop
@inproceedings{adaptivemisinformation,
  title={Defending against model stealing attacks with adaptive misinformation},
  author={Kariyappa, Sanjay and Qureshi, Moinuddin K},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={770--778},
  year={2020}
}

%accu drop
@article{pufNN,
  title={Defending against model extraction attacks with physical unclonable function},
  author={Li, Dawei and Liu, Di and Guo, Ying and Ren, Yangkun and Su, Jieyu and Liu, Jianwei},
  journal={Information Sciences},
  volume={628},
  pages={196--207},
  year={2023},
  publisher={Elsevier}
}

%% of detected adversarial examples
@article{aprotection,
  title={A protection against the extraction of neural network models},
  author={Chabanne, Herv{\'e} and Despiegel, Vincent and Guiga, Linda},
  journal={arXiv preprint arXiv:2005.12782},
  year={2020}
}

%Acci drop
@inproceedings{defendingagainst,
  title={Defending against neural network model stealing attacks using deceptive perturbations},
  author={Lee, Taesung and Edwards, Benjamin and Molloy, Ian and Su, Dong},
  booktitle={2019 IEEE Security and Privacy Workshops (SPW)},
  pages={43--49},
  year={2019},
  organization={IEEE}
}

%Performance
@inproceedings{preventingexfiltration,
  title={Preventing neural network model exfiltration in machine learning hardware accelerators},
  author={Isakov, Mihailo and Bu, Lake and Cheng, Hai and Kinsy, Michel A},
  booktitle={2018 Asian Hardware Oriented Security and Trust Symposium (AsianHOST)},
  pages={62--67},
  year={2018},
  organization={IEEE}
}

%https://dl.acm.org/doi/pdf/10.1145/3581783.3612515
@inproceedings{tan2023deep,
  title={Deep Neural Network Watermarking against Model Extraction Attack},
  author={Tan, Jingxuan and Zhong, Nan and Qian, Zhenxing and Zhang, Xinpeng and Li, Sheng},
  booktitle={Proceedings of the 31st ACM International Conference on Multimedia},
  pages={1588--1597},
  year={2023}
}

%search space
@inproceedings{telepathic,
  title={Telepathic headache: Mitigating cache side-channel attacks on convolutional neural networks},
  author={Chabanne, Herv{\'e} and Danger, Jean-Luc and Guiga, Linda and K{\"u}hne, Ulrich},
  booktitle={International Conference on Applied Cryptography and Network Security},
  pages={363--392},
  year={2021},
  organization={Springer}
}

%Accu drop, cosine simil, F2 score
@article{liang2024defending,
  title={Defending against model extraction attacks with OOD feature learning and decision boundary confusion},
  author={Liang, Chuang and Huang, Jie and Zhang, Zeping and Zhang, Shuaishuai},
  journal={Computers \& Security},
  volume={136},
  pages={103563},
  year={2024},
  publisher={Elsevier}
}


%First-order Tests on Variant-I
@article{guardingML,
  title={Guarding machine learning hardware against physical side-channel attacks},
  author={Dubey, Anuj and Cammarota, Rosario and Suresh, Vikram and Aysu, Aydin},
  journal={ACM Journal on Emerging Technologies in Computing Systems (JETC)},
  volume={18},
  number={3},
  pages={1--31},
  year={2022},
  publisher={ACM New York, NY}
}

%accuracy drop
@article{chaoticweights,
  title={Chaotic weights: A novel approach to protect intellectual property of deep neural networks},
  author={Lin, Ning and Chen, Xiaoming and Lu, Hang and Li, Xiaowei},
  journal={IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems},
  volume={40},
  number={7},
  pages={1327--1339},
  year={2020},
  publisher={IEEE}
}
@article{titcombe2021practical,
  title={Practical defences against model inversion attacks for split neural networks},
  author={Titcombe, Tom and Hall, Adam J and Papadopoulos, Pavlos and Romanini, Daniele},
  journal={arXiv preprint arXiv:2104.05743},
  year={2021}
}


%search space
@inproceedings{mitigating,
  title={Mitigating reverse engineering attacks on deep neural networks},
  author={Liu, Yuntao and Dachman-Soled, Dana and Srivastava, Ankur},
  booktitle={2019 IEEE Computer Society Annual Symposium on VLSI (ISVLSI)},
  pages={657--662},
  year={2019},
  organization={IEEE}
}

%model acc
@inproceedings{obfunas,
  title={ObfuNAS: A Neural Architecture Search-based DNN Obfuscation Approach},
  author={Zhou, Tong and Ren, Shaolei and Xu, Xiaolin},
  booktitle={Proceedings of the 41st IEEE/ACM International Conference on Computer-Aided Design},
  pages={1--9},
  year={2022}
}

%perf
@inproceedings{npufort,
  title={NPUFort: A secure architecture of DNN accelerator against model inversion attack},
  author={Wang, Xingbin and Hou, Rui and Zhu, Yifan and Zhang, Jun and Meng, Dan},
  booktitle={Proceedings of the 16th ACM International Conference on Computing Frontiers},
  pages={190--196},
  year={2019}
}

%ler

%acc loss
@inproceedings{dnncloak,
  title={DNNCloak: Secure DNN Models Against Memory Side-channel Based Reverse Engineering Attacks},
  author={Che, Yuezhi and Wang, Rujia},
  booktitle={2022 IEEE 40th International Conference on Computer Design (ICCD)},
  pages={89--96},
  year={2022},
  organization={IEEE}
}

%prob of correctly guessing
@inproceedings{deepring,
  title={DeepRing: Protecting deep neural network with blockchain},
  author={Goel, Akhil and Agarwal, Akshay and Vatsa, Mayank and Singh, Richa and Ratha, Nalini},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition workshops},
  pages={0--0},
  year={2019}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{mobilenet,
  title={Mobilenets: Efficient convolutional neural networks for mobile vision applications},
  author={Howard, Andrew G and Zhu, Menglong and Chen, Bo and Kalenichenko, Dmitry and Wang, Weijun and Weyand, Tobias and Andreetto, Marco and Adam, Hartwig},
  journal={arXiv preprint arXiv:1704.04861},
  year={2017}
}
@article{alexnet,
  title={Imagenet classification with deep convolutional neural networks},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  journal={Advances in neural information processing systems},
  volume={25},
  year={2012}
}
@inproceedings{shufflenet,
  title={Shufflenet: An extremely efficient convolutional neural network for mobile devices},
  author={Zhang, Xiangyu and Zhou, Xinyu and Lin, Mengxiao and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={6848--6856},
  year={2018}
}
@article{squeezenet,
  title={SqueezeNet: AlexNet-level accuracy with 50x fewer parameters and< 0.5 MB model size},
  author={Iandola, Forrest N and Han, Song and Moskewicz, Matthew W and Ashraf, Khalid and Dally, William J and Keutzer, Kurt},
  journal={arXiv preprint arXiv:1602.07360},
  year={2016}
}

@inproceedings{googlenet,
  title={Going deeper with convolutions},
  author={Szegedy, Christian and Liu, Wei and Jia, Yangqing and Sermanet, Pierre and Reed, Scott and Anguelov, Dragomir and Erhan, Dumitru and Vanhoucke, Vincent and Rabinovich, Andrew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1--9},
  year={2015}
}
@inproceedings{inception,
  title={Rethinking the inception architecture for computer vision},
  author={Szegedy, Christian and Vanhoucke, Vincent and Ioffe, Sergey and Shlens, Jon and Wojna, Zbigniew},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={2818--2826},
  year={2016}
}

@article{predictCR,
  title={Predicting the lossless compression ratio of remote sensing images with configurational entropy},
  author={Cheng, Xinghua and Li, Zhilin},
  journal={IEEE Journal of Selected Topics in Applied Earth Observations and Remote Sensing},
  volume={14},
  pages={11936--11953},
  year={2021},
  publisher={IEEE}
}

@article{mellin,
  title={A fast Mellin and scale transform},
  author={De Sena, Antonio and Rocchesso, Davide},
  journal={EURASIP Journal on Advances in Signal Processing},
  volume={2007},
  pages={1--9},
  year={2007},
  publisher={Springer}
}


@article{cover,
  title={Information theory and statistics},
  author={Cover, Thomas M and Thomas, Joy A},
  journal={Elements of information theory},
  volume={1},
  number={1},
  pages={279--335},
  year={1991},
  publisher={Wiley New York}
}

@inproceedings{entropy,
  title={Relating entropy theory to test data compression},
  author={Balakrishnan, Kedarnath J and Touba, Nur A},
  booktitle={Proceedings. Ninth IEEE European Test Symposium, 2004. ETS 2004.},
  pages={94--99},
  year={2004},
  organization={IEEE Computer Society}
}

@article{entropy2,
  title={Relationship between entropy and test data compression},
  author={Balakrishnan, Kedarnath J and Touba, Nur A},
  journal={IEEE Transactions on computer-aided design of integrated circuits and systems},
  volume={26},
  number={2},
  pages={386--395},
  year={2007},
  publisher={IEEE}
}


@inproceedings{lengthhiding,
  title={Hiding the lengths of encrypted messages via Gaussian padding},
  author={Degabriele, Jean Paul},
  booktitle={Proceedings of the 2021 ACM SIGSAC Conference on Computer and Communications Security},
  pages={1549--1565},
  year={2021}
}



@inproceedings{lengthhiding2,
  title={On hiding a plaintext length by preencryption},
  author={Tezcan, Cihangir and Vaudenay, Serge},
  booktitle={Applied Cryptography and Network Security: 9th International Conference, ACNS 2011, Nerja, Spain, June 7-10, 2011. Proceedings 9},
  pages={345--358},
  year={2011},
  organization={Springer}
}



@misc{KK1,
    title = {Samsung ex-employees leak tech firm’s DRAM secrets},
    url = {https://readwrite.com/samsung-ex-employees-leak-tech-firms-dram-secrets/},
    author = {Deanna Ritchie },
    year = {2023},
    note = {Accessed on 3 April, 2024}
}
%https://www.koreaherald.com/view.php?ud=20240103000777

@misc{KK2,
    title = {ASML claims an employee stole chip manufacturing secrets and sold them to China},
    url = {https://www.firstpost.com/world/asml-claims-an-employee-stole-chip-manufacturing-secrets-and-sold-them-to-china-12170742.html},
    author = { },
    publisher = {Firstpost},
    year = {2023},
    note = {Accessed on 3 April, 2024}
}

@misc{KK3,
    title = {Insider threats and their consequences},
    url = {https://www.ekransystem.com/en/blog/real-life-examples-insider-threat-caused-breaches},
    author = { Liudmyla Pryimenko},
    publisher = {Ekran},
    year = {Feb, 2024},
    note = {Accessed on 3 April, 2024}
}


@misc{KK4,
    title = {Samsung Fab Workers Leak Confidential Data While Using ChatGPT},
    url = {https://www.tomshardware.com/news/samsung-fab-workers-leak-confidential-data-to-chatgpt},
    author = {Anton Shilov },
    publisher = {Tom'sHardware},
    year = {April, 2023},
    note = {Accessed on 3 April, 2024}
}


@misc{SS1,
    title = {Data Security in the Age of Supercomputing},
    url = {https://medium.com/@cybertec/data-security-in-the-age-of-supercomputing-3b66464e54a0},
    author = { Jonathan Paulson },
     year = {Dec, 2023},
    note = {Accessed on 3 April, 2024}
}

%https://www.securityweek.com/ai-helps-crack-a-nist-recommended-post-quantum-encryption-algorithm/

@inproceedings{securelease,
  title={SecureLease: Maintaining Execution Control in The Wild using Intel SGX},
  author={Kumar, Sandeep and Panda, Abhisek and Sarangi, Smruti R},
  booktitle={Proceedings of the 23rd ACM/IFIP International Middleware Conference},
  pages={29--42},
  year={2022}
}



@misc{SCA,
    title = {Why side-channel analysis attacks are increasing and how to stop them},
    url = {https://www.ericsson.com/en/blog/2023/4/side-channel-analysis},
    author = {Niklas Lindskog and  Håkan Englund
Håkan Englund },
    publisher = {Ericsson blog},
    year = {April, 2023},
    note = {Accessed on 3 April, 2024}
}

@inproceedings{trafficSign1,
  title={Physical adversarial attacks on deep neural networks for traffic sign recognition: A feasibility study},
  author={Woitschek, Fabian and Schneider, Georg},
  booktitle={2021 IEEE Intelligent vehicles symposium (IV)},
  pages={481--487},
  year={2021},
  organization={IEEE}
}


@article{trafficSign2,
  title={Fooling a real car with adversarial traffic signs},
  author={Morgulis, Nir and Kreines, Alexander and Mendelowitz, Shachar and Weisglass, Yuval},
  journal={arXiv preprint arXiv:1907.00374},
  year={2019}
}

@inproceedings{trafficLight,
  title={Effects of and defenses against adversarial attacks on a traffic light classification CNN},
  author={Wan, Morris and Han, Meng and Li, Lin and Li, Zhigang and He, Selena},
  booktitle={Proceedings of the 2020 ACM Southeast Conference},
  pages={94--99},
  year={2020}
}

@article{KP,
  title={Adapting Kerckhoffs’s principle},
  author={Knoll, Thorsten},
  journal={Advanced Microkernel Operating Systems (2018)},
  volume={93},
  year={2018}
}

@article{squareful,
  title={On some properties of squarefree and squareful numbers},
  author={Mincu, Gabriel and Panaitopol, Lauren{\c{t}}iu},
  journal={Bulletin math{\'e}matique de la Soci{\'e}t{\'e} des Sciences Math{\'e}matiques de Roumanie},
  pages={63--68},
  year={2006},
  publisher={JSTOR}
}

@inproceedings{sgx,
  author = "Victor Costan and Srinivas Devadas",
  title = "Intel SGX Explained",
  year = "2016",
  booktitle = "Cryptology ePrint Archive, TechnicalReport086, MIT."
}

@article{puf,
  title={A puf taxonomy},
  author={McGrath, Thomas and Bagci, Ibrahim E and Wang, Zhiming M and Roedig, Utz and Young, Robert J},
  journal={Applied physics reviews},
  volume={6},
  number={1},
  year={2019},
  publisher={AIP Publishing}
}

@article{deepCompression,
  title={Deep compression: Compressing deep neural networks with pruning, trained quantization and huffman coding},
  author={Han, Song and Mao, Huizi and Dally, William J},
  journal={arXiv preprint arXiv:1510.00149},
  year={2015}
}

@article{pruned1,
  title={To prune, or not to prune: exploring the efficacy of pruning for model compression},
  author={Zhu, Michael and Gupta, Suyog},
  journal={arXiv preprint arXiv:1710.01878},
  year={2017}
}

@book{book,
author = {Smruti R. Sarangi},
title = {Next-Gen Computer Architecture},
date = {October 2023},
edition = {1st edition},
publisher={White Falcon},
isbn={8119510143} }


@incollection{SFC,
  title={Hilbert’s space-filling curve},
  author={Sagan, Hans},
  booktitle={Space-filling curves},
  pages={9--30},
  year={1994},
  publisher={Springer}
}

@article{surveyUncertainty,
  title={A survey of uncertainty in deep neural networks},
  author={Gawlikowski, Jakob and Tassi, Cedrique Rovile Njieutcheu and Ali, Mohsin and Lee, Jongseok and Humt, Matthias and Feng, Jianxiang and Kruspe, Anna and Triebel, Rudolph and Jung, Peter and Roscher, Ribana and others},
  journal={Artificial Intelligence Review},
  volume={56},
  number={Suppl 1},
  pages={1513--1589},
  year={2023},
  publisher={Springer}
}

@article{attestation,
  title={Supporting third party attestation for Intel SGX with Intel data center attestation primitives},
  author={Scarlata, Vinnie and Johnson, Simon and Beaney, James and Zmijewski, Piotr},
  journal={White paper},
  volume={12},
  year={2018},
  publisher={Intel Corporation}
}

@article{uniform1,
  title={The LUT-SR family of uniform random number generators for FPGA architectures},
  author={Thomas, David B and Luk, Wayne},
  journal={IEEE transactions on very large scale integration (vlsi) systems},
  volume={21},
  number={4},
  pages={761--770},
  year={2012},
  publisher={IEEE}
}

@inproceedings{uniform2,
  title={Fpga-optimised uniform random number generators using luts and shift registers},
  author={Thomas, David B and Luk, Wayne},
  booktitle={2010 International Conference on Field Programmable Logic and Applications},
  pages={77--82},
  year={2010},
  organization={IEEE}
}



@article{gaussian1,
  title={A Gaussian noise generator for hardware-based simulations},
  author={Lee, D-U and Luk, Wayne and Villasenor, John D and Cheung, Peter YK},
  journal={IEEE Transactions on Computers},
  volume={53},
  number={12},
  pages={1523--1534},
  year={2004},
  publisher={IEEE}
}

@article{gaussian2,
  title={Gaussian random number generation: A survey on hardware architectures},
  author={Malik, Jamshaid Sarwar and Hemani, Ahmed},
  journal={ACM Computing Surveys (CSUR)},
  volume={49},
  number={3},
  pages={1--37},
  year={2016},
  publisher={ACM New York, NY, USA}
}

@article{pchip,
  title={Hermite and piecewise cubic Hermite interpolation of fuzzy data},
  author={Zeinali, Masoumeh and Shahmorad, Sedaghat and Mirnia, Kamal},
  journal={Journal of Intelligent \& Fuzzy Systems},
  volume={26},
  number={6},
  pages={2889--2898},
  year={2014},
  publisher={IOS Press}
}

@misc{mellintr,
  title={The mellin transform},
  author={Bertrand, Jacqueline and Bertrand, Pierre and Ovarlez, Jean-Philippe},
  year={1995}
}

@inproceedings{massey,
  title={Guessing and entropy},
  author={Massey, James L},
  booktitle={Proceedings of 1994 IEEE International Symposium on Information Theory},
  pages={204},
  year={1994},
  organization={IEEE}
}

@article{noise,
  title={Noise immunity and robustness study of image recognition using a convolutional neural network},
  author={Ziyadinov, Vadim and Tereshonok, Maxim},
  journal={Sensors},
  volume={22},
  number={3},
  pages={1241},
  year={2022},
  publisher={MDPI}
}


@article{BPTest,
  title={A simple test for heteroscedasticity and random coefficient variation},
  author={Breusch, Trevor S and Pagan, Adrian R},
  journal={Econometrica: Journal of the econometric society},
  pages={1287--1294},
  year={1979},
  publisher={JSTOR}
}
@article{whiteTest,
  title={A heteroskedasticity-consistent covariance matrix estimator and a direct test for heteroskedasticity},
  author={White, Halbert},
  journal={Econometrica: journal of the Econometric Society},
  pages={817--838},
  year={1980},
  publisher={JSTOR}
}

@article{hmtt,
  title={HMTT: A hybrid hardware/software tracing system for bridging the DRAM access trace's semantic gap},
  author={Huang, Yongbing and Chen, Licheng and Cui, Zehan and Ruan, Yuan and Bao, Yungang and Chen, Mingyu and Sun, Ninghui},
  journal={ACM Transactions on Architecture and Code Optimization (TACO)},
  volume={11},
  number={1},
  pages={1--25},
  year={2014},
  publisher={ACM New York, NY, USA}
}


@inproceedings{neurobfuscator,
  title={Neurobfuscator: A full-stack obfuscation tool to mitigate neural architecture stealing},
  author={Li, Jingtao and He, Zhezhi and Rakin, Adnan Siraj and Fan, Deliang and Chakrabarti, Chaitali},
  booktitle={2021 IEEE International Symposium on Hardware Oriented Security and Trust (HOST)},
  pages={248--258},
  year={2021},
  organization={IEEE}
}

@article{geng2015optimal,
  title={Optimal noise adding mechanisms for approximate differential privacy},
  author={Geng, Quan and Viswanath, Pramod},
  journal={IEEE Transactions on Information Theory},
  volume={62},
  number={2},
  pages={952--969},
  year={2015},
  publisher={IEEE}
}

@inproceedings{nissim2007smooth,
  title={Smooth sensitivity and sampling in private data analysis},
  author={Nissim, Kobbi and Raskhodnikova, Sofya and Smith, Adam},
  booktitle={Proceedings of the thirty-ninth annual ACM symposium on Theory of computing},
  pages={75--84},
  year={2007}
}

@inproceedings{canales2024polynomial,
  title={Polynomial time cryptanalytic extraction of neural network models},
  author={Canales-Mart{\'\i}nez, Isaac A and Ch{\'a}vez-Saab, Jorge and Hambitzer, Anna and Rodr{\'\i}guez-Henr{\'\i}quez, Francisco and Satpute, Nitin and Shamir, Adi},
  booktitle={Annual International Conference on the Theory and Applications of Cryptographic Techniques},
  pages={3--33},
  year={2024},
  organization={Springer}
}

@inproceedings{carlini2020cryptanalytic,
  title={Cryptanalytic extraction of neural network models},
  author={Carlini, Nicholas and Jagielski, Matthew and Mironov, Ilya},
  booktitle={Annual international cryptology conference},
  pages={189--218},
  year={2020},
  organization={Springer}
}



@inproceedings{deutsch2023metior,
  title={Metior: A comprehensive model to evaluate obfuscating side-channel defense schemes},
  author={Deutsch, Peter W and Na, Weon Taek and Bourgeat, Thomas and Emer, Joel S and Yan, Mengjia},
  booktitle={Proceedings of the 50th Annual International Symposium on Computer Architecture},
  pages={1--16},
  year={2023}
}

@inproceedings{chakraborty2023randomized,
  title={Are randomized caches truly random? Formal analysis of randomized-partitioned caches},
  author={Chakraborty, Anirban and Bhattacharya, Sarani and Saha, Sayandeep and Mukhopadhyay, Debdeep},
  booktitle={2023 IEEE International Symposium on High-Performance Computer Architecture (HPCA)},
  pages={233--246},
  year={2023},
  organization={IEEE}
}

@inproceedings{samardzic2021f1,
  title={F1: A fast and programmable accelerator for fully homomorphic encryption},
  author={Samardzic, Nikola and Feldmann, Axel and Krastev, Aleksandar and Devadas, Srinivas and Dreslinski, Ronald and Peikert, Christopher and Sanchez, Daniel},
  booktitle={MICRO-54: 54th Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={238--252},
  year={2021}
}

@inproceedings{agrawal2023mad,
  title={MAD: Memory-Aware Design Techniques for Accelerating Fully Homomorphic Encryption},
  author={Agrawal, Rashmi and De Castro, Leo and Juvekar, Chiraag and Chandrakasan, Anantha and Vaikuntanathan, Vinod and Joshi, Ajay},
  booktitle={Proceedings of the 56th Annual IEEE/ACM International Symposium on Microarchitecture},
  pages={685--697},
  year={2023}
}


